ISCL: Interdependent Self-Cooperative Learning for Unpaired Image Denoising

With the advent of advances in self-supervised learning, paired clean-noisy data are no longer required in deep learning-based image denoising. However, existing blind denoising methods still require the assumption with regard to noise characteristics, such as zero-mean noise distribution and pixel-wise noise-signal independence; this hinders wide adaptation of the method in the medical domain. On the other hand, unpaired learning can overcome limitations related to the assumption on noise characteristics, which makes it more feasible for collecting the training data in real-world scenarios. In this paper, we propose a novel image denoising scheme, Interdependent Self-Cooperative Learning (ISCL), that leverages unpaired learning by combining cyclic adversarial learning with self-supervised residual learning. Unlike the existing unpaired image denoising methods relying on matching data distributions in different domains, the two architectures in ISCL, designed for different tasks, complement each other and boost the learning process. To assess the performance of the proposed method, we conducted extensive experiments in various biomedical image degradation scenarios, such as noise caused by physical characteristics of electron microscopy (EM) devices (film and charging noise), and structural noise found in low-dose computer tomography (CT). We demonstrate that the image quality of our method is superior to conventional and current state-of-the-art deep learning-based image denoising methods, including supervised learning.

==> reference.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{noise2self}
J.~Batson and L.~Royer, ``{N}oise2{S}elf: Blind denoising by
  self-supervision,'' in \emph{Proc. Int. Conf. Mach. Learn.}, Mar. 2019, pp.
  524--533.

\bibitem{redcnn}
H.~Chen, Y.~Zhang, M.~K. Kalra, F.~Lin, Y.~Chen, P.~Liao, J.~Zhou, and G.~Wang,
  ``Low-dose ct with a residual encoder-decoder convolutional neural network,''
  \emph{IEEE Trans. Med. Imag.}, vol.~36, no.~12, pp. 2524--2535, 2017.

\bibitem{cagan}
Z.~Huang, Z.~Chen, Q.~Zhang, G.~Quan, M.~Ji, C.~Zhang, Y.~Yang, X.~Liu,
  D.~Liang, H.~Zheng \emph{et~al.}, ``Cagan: a cycle-consistent generative
  adversarial network with attention for low-dose ct imaging,'' \emph{IEEE
  Trans. Comput. Imag.}, vol.~6, pp. 1203--1218, 2020.

\bibitem{hong2020end}
Z.~Hong, X.~Fan, T.~Jiang, and J.~Feng, ``End-to-end unpaired image denoising
  with conditional adversarial networks,'' in \emph{Proc. Assoc. Adv. Artific.
  Intell.}, Apr. 2020, pp. 4140--4149.

\bibitem{adn}
H.~Liao, W.-A. Lin, S.~K. Zhou, and J.~Luo, ``Adn: Artifact disentanglement
  network for unsupervised metal artifact reduction,'' \emph{IEEE Trans. Med.
  Imag.}, vol.~39, no.~3, pp. 634--643, 2019.

\bibitem{buades2005non}
A.~Buades, B.~Coll, and J.-M. Morel, ``A non-local algorithm for image
  denoising,'' in \emph{Proc. IEEE Comput. Soc. Conf. Comput. Vis. Pattern
  Recognit.}, vol.~2, Jun. 2005, pp. 60--65.

\bibitem{dabov2007}
K.~Dabov, A.~Foi, V.~Katkovnik, and K.~Egiazarian, ``Image denoising by sparse
  3-d transform-domain collaborative filtering,'' \emph{IEEE Trans. Image
  Process.}, vol.~16, no.~8, pp. 2080--2095, Aug. 2007.

\bibitem{mairal2009non}
J.~Mairal, F.~Bach, J.~Ponce, G.~Sapiro, and A.~Zisserman, ``Non-local sparse
  models for image restoration,'' in \emph{Proc. IEEE Int. Conf. Comput. Vis.},
  Sep. 2009, pp. 2272--2279.

\bibitem{bao2013fast}
C.~Bao, J.-F. Cai, and H.~Ji, ``Fast sparsity-based orthogonal dictionary
  learning for image restoration,'' in \emph{Proc. IEEE Int. Conf. Comput.
  Vis.}, Dec. 2013, pp. 3384--3391.

\bibitem{bao2015dictionary}
C.~Bao, H.~Ji, Y.~Quan, and Z.~Shen, ``Dictionary learning for sparse coding:
  Algorithms and convergence analysis,'' \emph{IEEE Trans. Pattern Anal. Mach.
  Intell.}, vol.~38, no.~7, pp. 1356--1369, Jul. 2016.

\bibitem{elad2006image}
M.~Elad and M.~Aharon, ``Image denoising via sparse and redundant
  representations over learned dictionaries,'' \emph{IEEE Trans. Image
  Process.}, vol.~15, no.~12, pp. 3736--3745, Dec. 2006.

\bibitem{papyan2017convolutional}
V.~Papyan, Y.~Romano, J.~Sulam, and M.~Elad, ``Convolutional dictionary
  learning via local processing,'' in \emph{Proc. IEEE Int. Conf. Comput.
  Vis.}, Oct. 2017, pp. 5296--5304.

\bibitem{vogel1996iterative}
C.~R. Vogel and M.~E. Oman, ``Iterative methods for total variation
  denoising,'' \emph{SIAM J. Sci. Comput.}, vol.~17, no.~1, pp. 227--238, Jan.
  1996.

\bibitem{vese2004image}
L.~A. Vese and S.~J. Osher, ``Image denoising and decomposition with total
  variation minimization and oscillatory functions,'' \emph{J. Math. Imaging
  Vis.}, vol.~20, no. 1-2, pp. 7--18, Jan. 2004.

\bibitem{getreuer2012rudin}
P.~Getreuer, ``Rudin-{O}sher-{F}atemi total variation denoising using split
  bregman,'' \emph{Image Process. On Line}, vol.~2, pp. 74--95, 2012.

\bibitem{zhang2017beyond}
K.~Zhang, W.~Zuo, Y.~Chen, D.~Meng, and L.~Zhang, ``Beyond a gaussian denoiser:
  Residual learning of deep cnn for image denoising,'' \emph{IEEE Trans. Image
  Process.}, vol.~26, no.~7, pp. 3142--3155, Jul. 2017.

\bibitem{lefkimmiatis2018universal}
S.~Lefkimmiatis, ``Universal denoising networks: a novel cnn architecture for
  image denoising,'' in \emph{Proc. IEEE conf. Comput. Vis. Pattern Recognit.},
  Jun. 2018, pp. 3204--3213.

\bibitem{noise2void}
A.~Krull, T.-O. Buchholz, and F.~Jug, ``Noise2void-learning denoising from
  single noisy images,'' in \emph{Proc. IEEE conf. Comput. Vis. Pattern
  Recognit.}, Jun. 2019, pp. 2129--2137.

\bibitem{quan2020self2self}
Y.~Quan, M.~Chen, T.~Pang, and H.~Ji, ``{S}elf2{S}elf with dropout: Learning
  self-supervised denoising from single image,'' in \emph{Proc. IEEE conf.
  Comput. Vis. Pattern Recognit.}, Jun. 2020, pp. 1890--1898.

\bibitem{hildebrand_gridtape_2017}
D.~G.~C. Hildebrand, B.~J. Graham, and W.-C.~A. Lee, ``Gridtape for fast
  nanoscale imaging,'' 2017.

\bibitem{graham_gridtape_2018}
B.~J. Graham, D.~G.~C. Hildebrand, and W.-C.~A. Lee, ``Gridtape imaging
  stage,'' 2018.

\bibitem{Graham657346}
\BIBentryALTinterwordspacing
B.~J. Graham, D.~G.~C. Hildebrand, A.~T. Kuan, J.~T. Maniates-Selvin, L.~A.
  Thomas, B.~L. Shanny, and W.-C.~A. Lee, ``High-throughput transmission
  electron microscopy with automated serial sectioning,'' \emph{bioRxiv}, 2019.
  [Online]. Available:
  \url{https://www.biorxiv.org/content/early/2019/06/02/657346}
\BIBentrySTDinterwordspacing

\bibitem{minh2019removing}
T.~Minh~Quan, D.~Grant Colburn~Hildebrand, K.~Lee, L.~A. Thomas, A.~T. Kuan,
  W.-C. Allen~Lee, and W.-K. Jeong, ``Removing imaging artifacts in electron
  microscopy using an asymmetrically cyclic adversarial network without paired
  training data,'' in \emph{Proc. IEEE Int. Conf. Comput. Vis. Workshop}, Oct.
  2019.

\bibitem{zhu2017unpaired}
J.-Y. Zhu, T.~Park, P.~Isola, and A.~A. Efros, ``Unpaired image-to-image
  translation using cycle-consistent adversarial networks,'' in \emph{Proc.
  IEEE Int. Conf. Comput. Vis.}, 2017, pp. 2223--2232.

\bibitem{jain2008natural}
V.~Jain and S.~Seung, ``Natural image denoising with convolutional networks,''
  \emph{Proc. Adv. Neural Inf. Process. Syst}, vol.~21, pp. 769--776, 2008.

\bibitem{burger2012image}
H.~C. Burger, C.~J. Schuler, and S.~Harmeling, ``Image denoising: Can plain
  neural networks compete with bm3d?'' in \emph{Proc. IEEE conf. Comput. Vis.
  Pattern Recognit.}\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2012, pp.
  2392--2399.

\bibitem{mao2016image}
X.~Mao, C.~Shen, and Y.-B. Yang, ``Image restoration using very deep
  convolutional encoder-decoder networks with symmetric skip connections,'' in
  \emph{Proc. Adv. Neural Inf. Process. Syst}, D.~D. Lee, M.~Sugiyama, U.~V.
  Luxburg, I.~Guyon, and R.~Garnett, Eds., 2016, pp. 2802--2810.

\bibitem{lefkimmiatis2017non}
S.~Lefkimmiatis, ``Non-local color image denoising with convolutional neural
  networks,'' in \emph{Proc. IEEE conf. Comput. Vis. Pattern Recognit.}, Jul.
  2017, pp. 3587--3596.

\bibitem{sacnn}
M.~Li, W.~Hsu, X.~Xie, J.~Cong, and W.~Gao, ``Sacnn: self-attention
  convolutional neural network for low-dose ct denoising with self-supervised
  perceptual loss network,'' \emph{IEEE Trans. Med. Imag.}, vol.~39, no.~7, pp.
  2289--2301, 2020.

\bibitem{he2016deep}
K.~He, X.~Zhang, S.~Ren, and J.~Sun, ``Deep residual learning for image
  recognition,'' in \emph{Proc. IEEE conf. Comput. Vis. Pattern Recognit.},
  2016, pp. 770--778.

\bibitem{batch-norm}
S.~Ioffe and C.~Szegedy, ``Batch normalization: Accelerating deep network
  training by reducing internal covariate shift,'' ser. Proc. Int. Conf. Mach.
  Learn., F.~Bach and D.~Blei, Eds., vol.~37, Lille, France, Jul. 2015, pp.
  448--456.

\bibitem{noise2noise}
J.~Lehtinen, J.~Munkberg, J.~Hasselgren, S.~Laine, T.~Karras, M.~Aittala, and
  T.~Aila, ``{N}oise2{N}oise: Learning image restoration without clean data,''
  in \emph{Proc. Int. Conf. Mach. Learn.}, J.~Dy and A.~Krause, Eds., vol.~80,
  Jul. 2018, pp. 2965--2974.

\bibitem{ulyanov2018deep}
D.~Ulyanov, A.~Vedaldi, and V.~Lempitsky, ``Deep image prior,'' in \emph{Proc.
  IEEE conf. Comput. Vis. Pattern Recognit.}, Jun. 2018, pp. 9446--9454.

\bibitem{cbdnet}
S.~Guo, Z.~Yan, K.~Zhang, W.~Zuo, and L.~Zhang, ``Toward convolutional blind
  denoising of real photographs,'' in \emph{Proc. IEEE conf. Comput. Vis.
  Pattern Recognit.}, 2019, pp. 1712--1722.

\bibitem{vdn}
Z.~Yue, H.~Yong, Q.~Zhao, D.~Meng, and L.~Zhang, ``Variational denoising
  network: Toward blind noise modeling and removal,'' in \emph{Proc. Adv.
  Neural Inf. Process. Syst}, vol.~32, 2019.

\bibitem{noise2sim}
\BIBentryALTinterwordspacing
C.~Niu and G.~Wang, ``Noise2sim--similarity-based self-learning for image
  denoising,'' 2020. [Online]. Available:
  \url{https://arxiv.org/abs/2011.03384}
\BIBentrySTDinterwordspacing

\bibitem{noise2kernel}
\BIBentryALTinterwordspacing
K.~Lee and W.-K. Jeong, ``Noise2kernel: Adaptive self-supervised blind
  denoising using a dilated convolutional kernel architecture,'' 2020.
  [Online]. Available: \url{https://arxiv.org/abs/2012.03623}
\BIBentrySTDinterwordspacing

\bibitem{chen2018image}
J.~Chen, J.~Chen, H.~Chao, and M.~Yang, ``Image blind denoising with generative
  adversarial network based noise modeling,'' in \emph{Proc. IEEE conf. Comput.
  Vis. Pattern Recognit.}, 2018, pp. 3155--3164.

\bibitem{park2019unpaired}
H.~S. Park, J.~Baek, S.~K. You, J.~K. Choi, and J.~K. Seo, ``Unpaired image
  denoising using a generative adversarial network in x-ray ct,'' \emph{IEEE
  Access}, vol.~7, pp. 110\,414--110\,425, 2019.

\bibitem{wu2020unpaired}
X.~Wu, M.~Liu, Y.~Cao, D.~Ren, and W.~Zuo, ``Unpaired learning of deep image
  denoising,'' in \emph{Eur. Conf. Comput. Vis.}\hskip 1em plus 0.5em minus
  0.4em\relax Springer, 2020, pp. 352--368.

\bibitem{drgan}
Y.~Huang, W.~Xia, Z.~Lu, Y.~Liu, H.~Chen, J.~Zhou, L.~Fang, and Y.~Zhang,
  ``Noise-powered disentangled representation for unsupervised speckle
  reduction of optical coherence tomography images,'' \emph{IEEE Trans. Med.
  Imag.}, 2020.

\bibitem{adain}
J.~Gu and J.~C. Ye, ``Adain-based tunable cyclegan for efficient unsupervised
  low-dose ct denoising,'' \emph{IEEE Trans. Comput. Imag.}, vol.~7, pp.
  73--85, 2021.

\bibitem{goodfellow2014generative}
I.~Goodfellow, J.~Pouget-Abadie, M.~Mirza, B.~Xu, D.~Warde-Farley, S.~Ozair,
  A.~Courville, and Y.~Bengio, ``Generative adversarial nets,'' in \emph{Proc.
  Adv. Neural Inf. Process. Syst}, 2014, pp. 2672--2680.

\bibitem{gulrajani2017improved}
I.~Gulrajani, F.~Ahmed, M.~Arjovsky, V.~Dumoulin, and A.~C. Courville,
  ``Improved training of wasserstein gans,'' in \emph{Proc. Adv. Neural Inf.
  Process. Syst}, 2017, pp. 5767--5777.

\bibitem{arjovsky2017wasserstein}
M.~Arjovsky, S.~Chintala, and L.~Bottou, ``{W}asserstein generative adversarial
  networks,'' in \emph{Proc. Int. Conf. Mach. Learn.}, vol.~70, Aug. 2017, pp.
  214--223.

\bibitem{lim2017geometric}
\BIBentryALTinterwordspacing
J.~H. Lim and J.~C. Ye, ``Geometric gan,'' 2017. [Online]. Available:
  \url{https://arxiv.org/abs/1705.02894}
\BIBentrySTDinterwordspacing

\bibitem{advattack}
D.~Bashkirova, B.~Usman, and K.~Saenko, ``Adversarial self-defense for
  cycle-consistent gans,'' in \emph{Proc. Adv. Neural Inf. Process. Syst},
  vol.~32, 2019.

\bibitem{han2018co}
B.~Han, Q.~Yao, X.~Yu, G.~Niu, M.~Xu, W.~Hu, I.~Tsang, and M.~Sugiyama,
  ``Co-teaching: Robust training of deep neural networks with extremely noisy
  labels,'' in \emph{Advances in neural information processing systems}, 2018,
  pp. 8527--8537.

\bibitem{SWA}
P.~Izmailov, D.~Podoprikhin, T.~Garipov, D.~Vetrov, and A.~G. Wilson,
  ``Averaging weights leads to wider optima and better generalization,''
  \emph{Assoc. Uncertainty Artific. Intell.}, 2018.

\bibitem{lookahead}
M.~Zhang, J.~Lucas, J.~Ba, and G.~E. Hinton, ``Lookahead optimizer: k steps
  forward, 1 step back,'' in \emph{Proc. Adv. Neural Inf. Process. Syst}, Dec.
  2019, pp. 9597--9608.

\bibitem{liu2019variance}
L.~Liu, H.~Jiang, P.~He, W.~Chen, X.~Liu, J.~Gao, and J.~Han, ``On the variance
  of the adaptive learning rate and beyond,'' \emph{Proc. Int. Conf. Learn.
  Represent}, 2020.

\bibitem{LDCT}
\BIBentryALTinterwordspacing
``Low dose ct grand challenge,'' 2016. [Online]. Available:
  \url{https://www.aapm.org/grandchallenge/}
\BIBentrySTDinterwordspacing

\bibitem{nam2018batch}
H.~Nam and H.-E. Kim, ``Batch-instance normalization for adaptively
  style-invariant neural networks,'' in \emph{Proc. Adv. Neural Inf. Process.
  Syst}, vol.~31, 2018, pp. 2558--2567.

\bibitem{ulyanov2016instance}
\BIBentryALTinterwordspacing
D.~Ulyanov, A.~Vedaldi, and V.~Lempitsky, ``Instance normalization: The missing
  ingredient for fast stylization,'' 2016. [Online]. Available:
  \url{https://arxiv.org/abs/1607.08022}
\BIBentrySTDinterwordspacing

\bibitem{long2015fully}
J.~Long, E.~Shelhamer, and T.~Darrell, ``Fully convolutional networks for
  semantic segmentation,'' in \emph{Proc. IEEE conf. Comput. Vis. Pattern
  Recognit.}, 2015, pp. 3431--3440.

\end{thebibliography}
